Local Algorithms for Sparse Spanning Graphs

Constructing a spanning tree of a graph is one of the most basic tasks in graph theory. We consider a relaxed version of this problem in the setting of local algorithms. The relaxation is that the constructed subgraph is a sparse spanning subgraph containing at most $(1+\epsilon)n$ edges (where $n$ is the number of vertices and $\epsilon$ is a given approximation/sparsity parameter). In the local setting, the goal is to quickly determine whether a given edge $e$ belongs to such a subgraph, without constructing the whole subgraph, but rather by inspecting (querying) the local neighborhood of $e$. The challenge is to maintain consistency. That is, to provide answers concerning different edges according to the same spanning subgraph. We first show that for general bounded-degree graphs, the query complexity of any such algorithm must be $\Omega(\sqrt{n})$. This lower bound holds for constant-degree graphs that have high expansion. Next we design an algorithm for (bounded-degree) graphs with high expansion, obtaining a result that roughly matches the lower bound. We then turn to study graphs that exclude a fixed minor (and are hence non-expanding). We design an algorithm for such graphs, which may have an unbounded maximum degree. The query complexity of this algorithm is $poly(1/\epsilon, h)$ (independent of $n$ and the maximum degree), where $h$ is the number of vertices in the excluded minor. Though our two algorithms are designed for very different types of graphs (and have very different complexities), on a high-level there are several similarities, and we highlight both the similarities and the differences.

==> lb.tex <==

In this section we prove the following theorem.
\BT\label{thm:lb}
Any local sparse spanning graph algorithm has query complexity $\Omega(\sqrt{n})$.
This result holds for graphs with a constant degree bound $d$ and for constant $0 \leq \eps \leq 2d/3$
and $0 \leq \delta < 1/3$.
\ET
%

Let $V$ be a set of vertices where $|V| = n$ and let $v_0$ and $v_1$ be a pair of distinct vertices in $V$.
In order to prove the lower bound we construct two families of $d$-regular graphs over $V$, $\calF^+_{(v_0, v_1)}$ and $\calF^-_{(v_0, v_1)}$.
$\calF^+_{(v_0, v_1)}$ is the family of $d$-regular graphs, $G=(V, E)$, for which $(v_0, v_1) \in E$.
$\calF^-_{(v_0, v_1)}$ is the family of $d$-regular for which $(v_0, v_1) \in E$ and
the removal of $(v_0, v_1)$ leaves the graph with two connected components, each of size~\footnote{Although a graph that is drawn uniformly from $\calF^+_{(v_0, v_1)}$ (or $\calF^-_{(v_0, v_1)}$) might be disconnected, this event happens with negligible probability~\cite{Bol01}.
Hence, the proof of the lower bound remains valid even if we consider $\calF^+_{(v_0, v_1)}\cap \calC$ and $\calF^-_{(v_0, v_1)}\cap\calC$ where $\calC$ is the family of connected graphs.}
$n/2$.
We prove that given $(v_0,v_1)$, any algorithm that performs at most $\sqrt{n}/c$ queries for some sufficiently large constant $c > 1$
cannot distinguish the case in which the graph is drawn uniformly at random from $\calF^+_{(v_0, v_1)}$ from the case in which the graph is drawn uniformly at random from $\calF^-_{(v_0, v_1)}$.
Essentially, if the number of queries is at most $\sqrt{n}/c$, then with high constant probability,
each new query to the graph returns a  new random vertex in both families. By ``new vertex'' we mean a vertex that neither  appeared in the query history nor in the answers history.
Since the algorithm must answer consistently with a connected graph $G'$, for every
graph in the support of $\calF^-_{(v_0, v_1)}$ it must answer positively on the query
$(v_0,v_1)$ (i.e., with probability $1$). But since the distributions on query-answer histories in both
cases are very close statistically, this can be shown to imply that there exist 
graphs for which the algorithm answers positively on a large fraction of the edges.
% \mnote{D: remember to deal with issue of connectivity of graphs.}





